Translate your gibberish: black-box adversarial attack on machine translation systems

Neural networks are deployed widely in natural language processing tasks on the industrial scale, and perhaps the most often they are used as compounds of automatic machine translation systems. In this work, we present a simple approach to fool state-of-the-art machine translation tools in the task of translation from Russian to English and vice versa. Using a novel black-box gradient-free tensor-based optimizer, we show that many online translation tools, such as Google, DeepL, and Yandex, may both produce wrong or offensive translations for nonsensical adversarial input queries and refuse to translate seemingly benign input phrases. This vulnerability may interfere with understanding a new language and simply worsen the user's experience while using machine translation systems, and, hence, additional improvements of these tools are required to establish better translation.

==> content/tmp.tex <==
\begin{figure}[t!]
\includegraphics[width=\textwidth]
    {figures/DeepL_attack4.png}
\caption{
    % The text
    Backtranslation results for the attack text 
    % ``the main goal of the Company is to provide the Company with the necessary information about the Company's activity in the future. The following information is important for the future of the company: the company's main activity is the activity of the person who is not a member of the company.''
    % is translated into Russian by DeepL translator incorrectly.
    ``\foreignlanguage{russian}{бёацсжю бгаьъэы гзйкщчж фйвьжиы дачэщйч бысёъгч ккзёйьи ккзёйьи гзйкщчж гбьъьиэ зсзгвлэ жьрцэъо гзйкщчж чтьёиэе рыьдяно рыьдяно фйвьжиы рыьдяно жьрэиэф щосющйе рыьдяно жаьйщсч рыьдяно жьрэиэф ъйлбмфь ъйлбмфь оощвишн быншийя бёацсжю бгаьъэы бреощее зжнмкьъ жаьйщсч ктлтксь ккзёйьи чъръпьм чъръпьм ъйлбмфь пдлешйщ быншийя ощуъиъв ыьбэъхс бёацсжю бгаьъэы бреощее зжнмкьъ жаьйщсч ктлтксь ккзёйьи}''.
    The resulting Russian translation has the following meaning in English:
    ``representative professional educator. Note''.
}
\label{fig:DeepL_attack4}
\end{figure}



% \mynote{actually we may underline that we do not generate adversarial examples per se (we arent aimed at misclassification), but rather generate inputs that are been translated though they should not}

% \mynote{TODO: Maybe add more criticism of zhang2021crafting and point out the differences in our approach.}

% \todopa{}{}{
% https://www.semanticscholar.org/paper/AdvAug\%3A-Robust-Adversarial-Augmentation-for-Neural-Cheng-Jiang/1e7d3a9846da556bc7b84ae1410d257b89448c30
% }

%\todopa{}{}{
%https://www.semanticscholar.org/paper/A-Targeted-Attack-on-Black-Box-Neural-Machine-with-Xu-Wang/2a46eb47e8742be29b16a5b83dc1a38616b24ce6
%}

%\todopa{}{}{https://www.semanticscholar.org/paper/PAEG\%3A-Phrase-level-Adversarial-Example-Generation-Wan-Yang/a6dd2a8debb5d5324c4f2be7fb7bb52ce109cbaf}

% \todopa{}{}{
% https://download.huan-zhang.com/events/srml2022/accepted/bhandari22lost.pdf
% }

%\todopa{}{}{http://fan-yao.com/paper/2021_SEED_nmtstroke.pdf}

% \todopa{}{}{https://arxiv.org/pdf/2303.01068v1.pdf}

%\todopa{kosinski2023theory}
%    {Theory of mind may have spontaneously emerged in large language models}
%    {https://arxiv.org/pdf/2302.02083.pdf}
%    {We can say that large language models are very clever now, etc...}

% \todopa{ebrahimi2018adversarial}
%     {On adversarial examples for character-level neural machine translation}
%     {https://arxiv.org/pdf/1806.09030.pdf}
%     {Very related work (see beamsearch in the text also)...}

% \todopa{zhang2021crafting}
%     {Crafting adversarial examples for neural machine translation}
%     {https://github.com/JHL-HUST/AdvNMT-WSLS}
%     {Very related work. See: ``Besides, WSLS exhibits strong transferability on attacking Baidu and Bing online translators.''}

% \todopa{sadrizadeh2023transfool}
%     {TransFool: An Adversarial Attack against Neural Machine Translation Models}
%     {https://arxiv.org/pdf/2302.00944.pdf}
%     {Very related work!}




% \begin{table}[t!]
% \caption{
%     Some examples for generated combinations of the hallucinogens for DeepL translator.
% }
% \label{tbl:results_DeepL_level2}
% \centering
% \begin{small}
% \renewcommand{\arraystretch}{1.0}
% \begin{tabular}{|p{0.9cm}|p{6cm}|p{6cm}|}\hline
% No & Text & Translation \\ \hline

% 1
% &
% \foreignlanguage{russian}{ъоэсйьл гзйкщчж гбьъьиэ жьрэиэф зжнмкьъ бысёъгч бреощее}
% &
% The following is an example of the following
% \\ \hline

% 2
% &
% \foreignlanguage{russian}{пдлешйщ фйвьжиы ккзёйьи гзйкщчж быншийя чтьёиэе ккзёйьи}
% &
% The first part of the story is the following
% \\ \hline

% 3
% &
% \foreignlanguage{russian}{жьрцэъо жьрцэъо ощуъиъв ъйлбмфь чтьёиэе ъйлбмфь зжнмкьъ}
% &
% Greetings from the Greetings Department of the Ministry of Foreign Affairs
% \\ \hline

% 4
% &
% \foreignlanguage{russian}{быншийя бгаьъэы ъоэсйьл чёхёшьч мжвлвфж рыьдяно гзйкщчж}
% &
% The formerly bogeyman is the one who is the most important person in the world.
% \\ \hline

% 5
% &
% \foreignlanguage{russian}{бреощее бысёъгч жаьйщсч жьрэиэф зсзгвлэ пдлешйщ оощвишн}
% &
% The main reason for this is that we have a lot of time and effort to get to the bottom of this
% \\ \hline

% \end{tabular}\end{small}\end{table}




% \begin{table}[t!]
% \caption{
%     Some examples for generated combinations of the hallucinogens for Google translator.
% }
% \label{tbl:results_google_level2}
% \centering
% \begin{small}
% \renewcommand{\arraystretch}{1.0}
% \begin{tabular}{|p{0.9cm}|p{6cm}|p{6cm}|}\hline
% No & Text & Translation \\ \hline

% 1
% &
% \foreignlanguage{russian}{уясъцёь ъыллщьн пщмёжны ъныуазу йтдкцяе бщагчёщ ъёефнся}
% &
% understanding of the bang
% \\ \hline

% 2
% &
% \foreignlanguage{russian}{быошийя ъёефнся ъбывзлц ъжлхчлы быошийя йтдкцяе пёвюмыц}
% &
% I would have been the bungles of Kommersant Kommersant
% \\ \hline

% 3
% &
% \foreignlanguage{russian}{вытёщдч доцшлны гфоаььн пёвюмыц бяёщжии ътшлшэь ъфоъкцж}
% &
% Stepschdch is an ahead of the National Academy of Education
% \\ \hline

% 4
% &
% \foreignlanguage{russian}{уясъцёь дщижщяп штшнлхж пщмёжны пёвюмыц ъныуазу ъокнёйф}
% &
% understanding of the throat of the stamp
% \\ \hline

% 5
% &
% \foreignlanguage{russian}{вытёщдч доцшлны ъувщжёь бйввкшя пщмёжны ъыллщьн бяёщжии}
% &
% The priests of the Associate Professor Kommersant
% \\ \hline

% \end{tabular}\end{small}\end{table}




% \begin{table}[t!]
% \caption{
%     Some examples for generated combinations of the hallucinogens for Yandex translator.
% }
% \label{tbl:results_yandex_level2}
% \centering
% \begin{small}
% \renewcommand{\arraystretch}{1.0}
% \begin{tabular}{|p{0.9cm}|p{6cm}|p{6cm}|}\hline
% No & Text & Translation \\ \hline

% 1
% &
% \foreignlanguage{russian}{мощыъпз щаафечу йьаёьеб ощуъиъв нзеъёаь ощуъиъв иысвщёы}
% &
% The power of the heart is now being felt by the heart of the heart .
% \\ \hline

% 2
% &
% \foreignlanguage{russian}{иысвщёы ъяляужь ощуъиъв мощыъпз ъныуазу ущйинъу ъныуазу}
% &
% and you will feel the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the power of the
% \\ \hline

% 3
% &
% \foreignlanguage{russian}{ъяляужь иысвщёы иьллтёу оэеыъьё щаафечу мощыъпз ощуъиъв}
% &
% I will be able to feel the power of the heart.
% \\ \hline

% 4
% &
% \foreignlanguage{russian}{бьвтюья иысвщёы бьвтюья здблоьп щаафечу шэьдкйя доцшлмь}
% &
% I'm sorry, I 'm sorry , I 'm sorry , I 'm sorry , I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry, I 'm sorry.
% \\ \hline

% 5
% &
% \foreignlanguage{russian}{ощуъиъв доцшлмь ъныуазу онуьлйц ьвднэйу здблоьп ьвднэйу}
% &
% I feel like I 'm on the right side of the right side of the right side of the right side of the right side of the right side of the right side
% \\ \hline

% \end{tabular}\end{small}\end{table}




% \mynote{TODO: its questionable if we need manual examples from below}

% We present below some examples of gibberish text in Russian translatable by  DeepL:
% \begin{enumerate}
%     \item 
%         The combination of the hallucinogens
%         ``\foreignlanguage{russian}{фйвьжиы фйвьжиы пдлешйщ ккзёйьи гбьъьиэ жцчыщцй ктлтксь ыьбэъхс ъоэсйьл жьрцэъо мжвлвфж гзйкщчж жцчыщцй щосющйе ккзёйьи ккзёйьи фйвьжиы быншийя дачэщйч бысёъгч бёацсжю бысёъгч жцчыщцй жьрэиэф гмххъьн бёацсжю бгаьъэы чёхёшьч оощвишн бжкльлш бжкльлш щосющйе бгаьъэы дачэщйч ъоэсйьл пдлешйщ жцчыщцй жаьйщсч ъоэсйьл чёхёшьч бреощее ъйлбмфь бреощее бгаьъэы бжкльлш жьрэиэф ктлтксь ктлтксь бгаьъэы}''
%         leads to the English text and related translation, which are presented in Figure~\ref{fig:DeepL_attack1};
%     \item 
%         The combination of the hallucinogens
%         ``\foreignlanguage{russian}{бёацсжю бгаьъэы гзйкщчж фйвьжиы дачэщйч бысёъгч ккзёйьи ъоэсйьл гзйкщчж гбьъьиэ жьрэиэф зжнмкьъ бысёъгч бреощее жьрцэъо быелръъ жаьйщсч бреощее зжнмкьъ чъръпьм ъйлбмфь ккзёйьи гзйкщчж гбьъьиэ зсзгвлэ жьрцэъо гзйкщчж чтьёиэе бысёъгч жцчыщцй жьрэиэф гмххъьн бёацсжю бгаьъэы чёхёшьч чёхёшьч ктлтксь бысёъгч ъоэсйьл быелръъ чёхёшьч гмххъьн жьрэиэф бжкльлш зсзгвлэ жьрцэъо бысёъгч бысёъгч бжкльлш}''
%         leads to the English text and related translation, which are presented in Figure~\ref{fig:DeepL_attack2};
%     \item 
%         The combination of the hallucinogens
%         ``\foreignlanguage{russian}{рыьдяно рыьдяно фйвьжиы рыьдяно жьрэиэф щосющйе рыьдяно жцчыщцй фйвьжиы гбьъьиэ зсзгвлэ бгаьъэы рыьдяно ккзёйьи ктлтксь бфзскйт щосющйе пдлешйщ мжвлвфж рыьдяно гзйкщчж зсзгвлэ гзйкщчж гзйкщчж гбьъьиэ оощвишн гзйкщчж чёхёшьч пдлешйщ жцчыщцй жаьйщсч ъоэсйьл чёхёшьч бреощее ъйлбмфь ктлтксь бфзскйт щосющйе пдлешйщ мжвлвфж рыьдяно гзйкщчж чъръпьм чъръпьм ъйлбмфь пдлешйщ быншийя ощуъиъв ыьбэъхс}''
%         leads to the English text and related translation, which are presented in Figure~\ref{fig:DeepL_attack3};
%     \item 
%         The combination of the hallucinogens
%         ``\foreignlanguage{russian}{бёацсжю бгаьъэы гзйкщчж фйвьжиы дачэщйч бысёъгч ккзёйьи ккзёйьи гзйкщчж гбьъьиэ зсзгвлэ жьрцэъо гзйкщчж чтьёиэе рыьдяно рыьдяно фйвьжиы рыьдяно жьрэиэф щосющйе рыьдяно жаьйщсч рыьдяно жьрэиэф ъйлбмфь ъйлбмфь оощвишн быншийя бёацсжю бгаьъэы бреощее зжнмкьъ жаьйщсч ктлтксь ккзёйьи чъръпьм чъръпьм ъйлбмфь пдлешйщ быншийя ощуъиъв ыьбэъхс бёацсжю бгаьъэы бреощее зжнмкьъ жаьйщсч ктлтксь ккзёйьи}''
%         leads to the English text and related translation, which are presented in Figure~\ref{fig:DeepL_attack4};
%     \item 
%         The combination of the hallucinogens
%         ``\foreignlanguage{russian}{бёацсжю бгаьъэы гзйкщчж фйвьжиы дачэщйч бысёъгч ккзёйьи чёхёшьч ктлтксь бысёъгч ъоэсйьл быелръъ чёхёшьч гмххъьн ъоэсйьл ккзёйьи бжкльлш пдлешйщ рыьдяно жьрцэъо пдлешйщ бёацсжю зсзгвлэ бёацсжю чтьёиэе быншийя бжкльлш гзйкщчж чъръпьм чъръпьм ъйлбмфь пдлешйщ быншийя ощуъиъв ыьбэъхс бёацсжю бгаьъэы бреощее зжнмкьъ жаьйщсч ктлтксь ккзёйьи оощвишн бжкльлш бжкльлш щосющйе бгаьъэы дачэщйч ъоэсйьл}''
%         leads to the English text and related translation, which are presented in Figure~\ref{fig:DeepL_attack5}.
% \end{enumerate}


% \begin{table}[t!]
% \caption{
%     The top-$33$ generated hallucinogens for DeepL translator.
% }
% \label{tbl:results_DeepL_level1}
% \centering
% \begin{small}
% \renewcommand{\arraystretch}{1.0}
% % \fontsize{10pt}{11pt}
% % \selectfont
% % \setlength{\tabcolsep}{5pt}
% \begin{tabular}{|p{0.8cm}|p{1.9cm}|p{4.7cm}|p{4.7cm}|}
% \toprule
% No & Loss value & Text & Translation \\
% \midrule
% % Autogenerated results for "DeepL" (level 1)
%  1 & -42.52 & \foreignlanguage{russian}{быелръъ} & formerly \\ \hline
%  2 & -39.47 & \foreignlanguage{russian}{пдлешйщ} & Synopsis: \\ \hline
%  3 & -38.53 & \foreignlanguage{russian}{бысёъгч} & Quickly \\ \hline
%  4 & -37.20 & \foreignlanguage{russian}{чтьёиэе} & READ MORE \\ \hline
%  5 & -34.84 & \foreignlanguage{russian}{щосющйе} & Synopsis: \\ \hline
%  6 & -34.84 & \foreignlanguage{russian}{быншийя} & former \\ \hline
%  7 & -30.42 & \foreignlanguage{russian}{зсзгвлэ} & ssgvle \\ \hline
%  8 & -30.12 & \foreignlanguage{russian}{бгаьъэы} & bgaiy \\ \hline
%  9 & -27.67 & \foreignlanguage{russian}{дачэщйч} & Dachshund \\ \hline
% 10 & -27.50 & \foreignlanguage{russian}{бреощее} & Breaking \\ \hline
% 11 & -27.21 & \foreignlanguage{russian}{бжкльлш} & bjklsh \\ \hline
% 12 & -26.86 & \foreignlanguage{russian}{оощвишн} & Promotion \\ \hline
% 13 & -25.08 & \foreignlanguage{russian}{ощуъиъв} & Feelings \\ \hline
% 14 & -24.08 & \foreignlanguage{russian}{гбьъьиэ} & gbjie \\ \hline
% 15 & -24.07 & \foreignlanguage{russian}{рыьдяно} & snarky \\ \hline
% 16 & -23.64 & \foreignlanguage{russian}{жьрэиэф} & zhreif \\ \hline
% 17 & -23.64 & \foreignlanguage{russian}{жцчыщцй} & Žučičky \\ \hline
% 18 & -23.49 & \foreignlanguage{russian}{чёхёшьч} & What the fuck \\ \hline
% 19 & -23.37 & \foreignlanguage{russian}{зжнмкьъ} & zznnmkj \\ \hline
% 20 & -23.21 & \foreignlanguage{russian}{гмххъьн} & gmhxjn \\ \hline
% 21 & -23.19 & \foreignlanguage{russian}{жьрцэъо} & Jrceo \\ \hline
% 22 & -23.15 & \foreignlanguage{russian}{бёацсжю} & boatsjue \\ \hline
% 23 & -23.04 & \foreignlanguage{russian}{гзйкщчж} & gzcjcj \\ \hline
% 24 & -22.33 & \foreignlanguage{russian}{ъоэсйьл} & Yoesyl \\ \hline
% 25 & -22.00 & \foreignlanguage{russian}{мжвлвфж} & mjvlvfj \\ \hline
% 26 & -21.61 & \foreignlanguage{russian}{ктлтксь} & ktltx \\ \hline
% 27 & -21.38 & \foreignlanguage{russian}{фйвьжиы} & fyvji \\ \hline
% 28 & -21.25 & \foreignlanguage{russian}{жаьйщсч} & zhayshch \\ \hline
% 29 & -20.78 & \foreignlanguage{russian}{ккзёйьи} & kkzoyi \\ \hline
% 30 & -20.66 & \foreignlanguage{russian}{бфзскйт} & bfzskyt \\ \hline
% 31 & -20.47 & \foreignlanguage{russian}{ыьбэъхс} & yybexx \\ \hline
% 32 & -20.27 & \foreignlanguage{russian}{ъйлбмфь} & ylbmfj \\ \hline
% 33 & -20.23 & \foreignlanguage{russian}{чъръпьм} & chirp \\
% \bottomrule
% \end{tabular}\end{small}\end{table}

% \begin{table}[t!]
% \caption{
%     The top-$33$ generated hallucinogens for Google translator.
% }
% \label{tbl:results_google_level1}
% \centering
% \begin{small}
% \renewcommand{\arraystretch}{1.0}
% \begin{tabular}{|p{0.8cm}|p{1.9cm}|p{4.7cm}|p{4.7cm}|}\hline
% No & Loss value & Text & Translation \\ \hline
% % Autogenerated results for "google" (level 1)
%  1 & -50.18 & \foreignlanguage{russian}{ъувщжёь} & Knight \\ \hline
%  2 & -48.27 & \foreignlanguage{russian}{бйввкшя} & Former \\ \hline
%  3 & -45.13 & \foreignlanguage{russian}{дщижщяп} & Building \\ \hline
%  4 & -43.64 & \foreignlanguage{russian}{мощыъпз} & Power \\ \hline
%  5 & -43.38 & \foreignlanguage{russian}{ъыьгрвх} & Kommersant \\ \hline
%  6 & -41.73 & \foreignlanguage{russian}{пёвюмыц} & first \\ \hline
%  7 & -41.19 & \foreignlanguage{russian}{ъёефнся} & Currently \\ \hline
%  8 & -37.32 & \foreignlanguage{russian}{ъжлхчлы} & Kommersant \\ \hline
%  9 & -37.21 & \foreignlanguage{russian}{ъоэсйьл} & Kommersant \\ \hline
% 10 & -37.05 & \foreignlanguage{russian}{вытёщдч} & priest \\ \hline
% 11 & -36.29 & \foreignlanguage{russian}{бщагчёщ} & Passing \\ \hline
% 12 & -35.53 & \foreignlanguage{russian}{штшнлхж} & Stitch \\ \hline
% 13 & -33.98 & \foreignlanguage{russian}{гяшрьнп} & Gagarin \\ \hline
% 14 & -33.39 & \foreignlanguage{russian}{здкънсп} & health \\ \hline
% 15 & -32.24 & \foreignlanguage{russian}{ъыллщьн} & Kommersant \\ \hline
% 16 & -32.00 & \foreignlanguage{russian}{ътшлшэь} & Kommersant \\ \hline
% 17 & -31.81 & \foreignlanguage{russian}{быошийя} & To be \\ \hline
% 18 & -31.69 & \foreignlanguage{russian}{доцшлны} & Associated \\ \hline
% 19 & -31.62 & \foreignlanguage{russian}{пщмёжны} & They are \\ \hline
% 20 & -31.38 & \foreignlanguage{russian}{ъухвмгс} & Kommersant \\ \hline
% 21 & -30.80 & \foreignlanguage{russian}{ъбывзлц} & Kommersant \\ \hline
% 22 & -30.24 & \foreignlanguage{russian}{бяёщжии} & beads \\ \hline
% 23 & -30.15 & \foreignlanguage{russian}{ъокнёйф} & Continuity \\ \hline
% 24 & -30.10 & \foreignlanguage{russian}{ъфъыхлч} & Kommersant \\ \hline
% 25 & -30.09 & \foreignlanguage{russian}{птйдфдц} & PTDDC \\ \hline
% 26 & -29.54 & \foreignlanguage{russian}{йтдкцяе} & induction \\ \hline
% 27 & -29.29 & \foreignlanguage{russian}{уясъцёь} & understanding \\ \hline
% 28 & -29.28 & \foreignlanguage{russian}{зсзгвлэ} & ZSZGLE \\ \hline
% 29 & -29.01 & \foreignlanguage{russian}{ъфоъкцж} & Kommersant \\ \hline
% 30 & -28.97 & \foreignlanguage{russian}{жхнаеыь} & grunts \\ \hline
% 31 & -28.68 & \foreignlanguage{russian}{ъфкщтнэ} & Kommersant \\ \hline
% 32 & -28.47 & \foreignlanguage{russian}{ъныуазу} & Kommersant \\ \hline
% 33 & -28.38 & \foreignlanguage{russian}{гфоаььн} & fifajn \\ \hline
% \end{tabular}\end{small}\end{table}




% \begin{table}[t!]
% \caption{
%     The top-$33$ generated hallucinogens for Yandex translator.
% }
% \label{tbl:results_yandex_level1}
% \centering
% \begin{small}
% \renewcommand{\arraystretch}{1.0}
% \begin{tabular}{|p{0.8cm}|p{1.9cm}|p{4.7cm}|p{4.7cm}|}\hline
% No & Loss value & Text & Translation \\ \hline
% % Autogenerated results for "yandex" (level 1)
%  1 & -42.87 & \foreignlanguage{russian}{здблоьп} & hello \\ \hline
%  2 & -42.15 & \foreignlanguage{russian}{ьвднэйу} & Today \\ \hline
%  3 & -40.44 & \foreignlanguage{russian}{онуьлйц} & online \\ \hline
%  4 & -35.26 & \foreignlanguage{russian}{смэёыюш} & see also \\ \hline
%  5 & -34.94 & \foreignlanguage{russian}{иысвщёы} & and more \\ \hline
%  6 & -32.76 & \foreignlanguage{russian}{схисеъм} & scheme \\ \hline
%  7 & -31.20 & \foreignlanguage{russian}{мощыъпз} & The power of the \\ \hline
%  8 & -30.76 & \foreignlanguage{russian}{кццжйхк} & kccjhk \\ \hline
%  9 & -30.54 & \foreignlanguage{russian}{ътшмщэь} & kommersant \\ \hline
% 10 & -27.58 & \foreignlanguage{russian}{ъубщжёь} & kommersant \\ \hline
% 11 & -27.56 & \foreignlanguage{russian}{ъььгрвх} & ygrvh \\ \hline
% 12 & -27.48 & \foreignlanguage{russian}{кмтсгфк} & kmtsgfc \\ \hline
% 13 & -27.08 & \foreignlanguage{russian}{иощсцйм} & ioschcym \\ \hline
% 14 & -26.32 & \foreignlanguage{russian}{нзеъёаь} & nzeea \\ \hline
% 15 & -26.10 & \foreignlanguage{russian}{бмъчкьь} & bmchk \\ \hline
% 16 & -25.67 & \foreignlanguage{russian}{ъоэсйьм} & yoesm \\ \hline
% 17 & -25.56 & \foreignlanguage{russian}{ъыклщьн} & kommersant \\ \hline
% 18 & -25.49 & \foreignlanguage{russian}{бьвтюья} & byuya \\ \hline
% 19 & -25.48 & \foreignlanguage{russian}{иьеьрёъ} & iyere \\ \hline
% 20 & -25.22 & \foreignlanguage{russian}{ущйинъу} & pinyin \\ \hline
% 21 & -24.49 & \foreignlanguage{russian}{шэьдкйя} & shadkya \\ \hline
% 22 & -24.03 & \foreignlanguage{russian}{ощуъиъв} & feeling \\ \hline
% 23 & -24.03 & \foreignlanguage{russian}{иьллтёу} & illteu \\ \hline
% 24 & -23.68 & \foreignlanguage{russian}{щаафечу} & right now \\ \hline
% 25 & -23.41 & \foreignlanguage{russian}{ъяляужь} & for the service \\ \hline
% 26 & -23.33 & \foreignlanguage{russian}{нмьрщшт} & nmrsht \\ \hline
% 27 & -23.16 & \foreignlanguage{russian}{оэеыъьё} & oeeye \\ \hline
% 28 & -23.10 & \foreignlanguage{russian}{йьаёьеб} & yaeeb \\ \hline
% 29 & -22.72 & \foreignlanguage{russian}{флжсйид} & fljsyid \\ \hline
% 30 & -22.67 & \foreignlanguage{russian}{пёыэулм} & peeulm \\ \hline
% 31 & -22.59 & \foreignlanguage{russian}{бдлпроь} & bdlpro \\ \hline
% 32 & -22.56 & \foreignlanguage{russian}{доцшлмь} & assoc . \\ \hline
% 33 & -22.53 & \foreignlanguage{russian}{ъныуазу} & kommersant \\ \hline
% \end{tabular}\end{small}\end{table}


==> helpers/demo_from_template.tex <==
% For russian (TODO: check). T1 fonts will be used to generate the final print and online PDFs, so please use T1 fonts in your manuscript whenever possible. Other font encondings may result in incorrect characters.
%
%
%
\section{First Section}
\subsection{A Subsection Sample}
Please note that the first paragraph of a section or subsection is
not indented. The first paragraph that follows a table, figure,
equation etc. does not need an indent, either.

Subsequent paragraphs, however, are indented.

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
\includegraphics[width=\textwidth]{figures/fig1.eps}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}

%For citations of references, we prefer the use of square brackets
%and consecutive numbers. Citations using labels or the author/year
%convention are also acceptable. The following bibliography provides
%a sample reference list with entries for journal
%articles~\cite{ref_article1}, an LNCS %chapter~\cite{ref_lncs1}, a
%book~\cite{ref_book1}, proceedings without editors~\cite{ref_proc1},
%and a homepage~\cite{ref_url1}. Multiple citations are grouped
%\cite{ref_article1,ref_lncs1,ref_book1},
%\cite{ref_article1,ref_book1,ref_proc1,ref_url1}.



%\begin{thebibliography}{8}
%\bibitem{ref_article1}
%Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

%\bibitem{ref_lncs1}
%Author, F., Author, S.: Title of a proceedings paper. In: Editor,
%F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
%Springer, Heidelberg (2016). \doi{10.10007/1234567890}

%\bibitem{ref_book1}
%Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
%Location (1999)

%\bibitem{ref_proc1}
%Author, A.-B.: Contribution title. In: 9th International Proceedings
%on Proceedings, pp. 1--2. Publisher, Location (2010)

%\bibitem{ref_url1}
%LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
%Oct 2017
%\end{thebibliography}
